On the Stability of Approximate Message Passing with Independent Measurement Ensembles

Approximate message passing (AMP) is a scalable, iterative approach to signal recovery. For structured random measurement ensembles, including independent and identically distributed (i.i.d.) Gaussian and rotationally-invariant matrices, the performance of AMP can be characterized by a scalar recursion called state evolution (SE). The pseudo-Lipschitz (polynomial) smoothness is conventionally assumed. In this work, we extend the SE for AMP to a new class of measurement matrices with independent (not necessarily identically distributed) entries. We also extend it to a general class of functions, called controlled functions which are not constrained by the polynomial smoothness; unlike the pseudo-Lipschitz function that has polynomial smoothness, the controlled function grows exponentially. The lack of structure in the assumed measurement ensembles is addressed by leveraging Lindeberg-Feller. The lack of smoothness of the assumed controlled function is addressed by a proposed conditioning technique leveraging the empirical statistics of the AMP instances. The resultants grant the use of the SE to a broader class of measurement ensembles and a new class of functions.

==> Intro2.tex <==
\section{Introduction}
\label{secI}	
	%%
        The problem of signal recovery from a linear observation 
        \begin{equation}
         \label{eq:5}
            \by = \bA\bx_0 +\bw
        \end{equation} 
        appears in various fields \cite{Kay97,Donoho2006,Schniter2022}, where $\by \in \R^{n \times 1}$, $\bA \in \R^{n \times N}$ is a given measurement matrix, $\bx_0 \in \R^{N \times 1}$ is the signal to be recovered, and $\bw \in \R^{n \times 1}$ is an additive noise. 
	%%
        Of particular interest is the case when $\bA$ is overcomplete ($n \ll N$), in which the number of observations is strictly smaller than the number of reconstruction variables.    
	%%
        The computational cost to solve this problem is typically prohibitive when the dimensions $n$ and $N$ become large, which has been motivating low-cost approaches. 
	%%
	
	%%
        Message passing represents one of the most important progress in inference which can be applied to handle the large-dimensionality of the problem. 
        %%
        It provides a practically affordable means to approach the minimum mean square error (MMSE) or the channel capacity promised by information theory.
        %%
        Conventionally, sparsity is essential for message passing, in the form of sparse connection and  sparse signaling \cite{Richarson2001}.
        %%
        Recently, the approximate message-passing (AMP) algorithm has received significant attention \cite{Donoho2009,Donoho2010,Donoho20102}; it performs excellently in systems that are dense in both the measurement matrix $\bA$ (connection) and the $\bx_0$ (signalling). 
        %%
     
     %
    % The remarkable features of AMP have inspired a wide range of applications such as low-rank matrix estimation \cite{Montanari2017,Fletcher2018,Lesieur2017}, generalized linear models \cite{Rangan11,Snicher2012,Mondelli2021}, deep learning \cite{Pandit2019,Pandit2020,Emami2020}, multiple-input multiple-output (MIMO) detection \cite{Zhang8, Jeon2, Schniter2010}, MIMO channel estimation \cite{Kim2015,Bellili2018,baron2020}, radar signal processing \cite{Huang2016,Jiang2019, Zheng2017}, and compressive imaging \cite{Sung3, Tan2015, Millard2020}. 
    %%
    The remarkable features of AMP have inspired a wide range of applications such as low-rank matrix estimation \cite{Montanari2017,Fletcher2018,Lesieur2017}, deep learning \cite{Pandit2019,Pandit2020,Emami2020}, multiple-input multiple-output (MIMO) detection \cite{Zhang8, Jeon2, Schniter2010}, MIMO channel estimation \cite{Kim2015,Bellili2018,baron2020}, and compressive imaging \cite{Sung3, Tan2015, Millard2020}. 
    %%
    Despite of its widespread applicability, the AMP algorithm suffers from instability; it requires a special structure of measurement matrices. 
    %%
    When the matrix $\bA$ is ill-conditioned or has non-zero mean entries \cite{Caltagirone2014,Ma2017,Sundeep19}, the AMP recursion may diverge, which is closely related to the dynamic of AMP induced by the structure of the random measurement ensembles. 
    %%
    Understanding the dynamics of AMP for different classes of random measurement matrix $\bA$ has been an outstanding open problem.	
    \subsection{Related Works}
    %%
    The most widely studied random measurement ensemble is the $\bA$ with the independent and identically distributed (i.i.d.) zero-mean and $\frac{1}{n}$-variance Gaussian entries. 
    %%
    Under this assumption, the first rigorous description of the state evolution (SE) for AMP is due to Bayati and Montanari \cite{Bayati11}. 
    %%
    As the dimensions $n$ and $N$ tend to infinity while $\frac{n}{N}$ is kept being constant, the mean squared error (MSE) performance of AMP can be  asymptotically characterized by SE. 
    %%
    Particularly, the AMP algorithm converges to the MMSE estimator given the distributions of the signal $\bx_0$ and noise $\bw$ known a priori.  
    %%
    Under the same Gaussian $\bA$ as in \cite{Bayati11}, Rush \emph{et. al} \cite{Rush2018} showed non-asymptotic results for AMP with finite $n$ and $N$, revealing that the probability of deviation from the SE prediction decays exponentially in $n$. 
    %%

    %%
    The remarkable features of AMP have inspired extensive research efforts on characterizing SE for different measurement ensembles such as sub-Gaussian $\bA$ by Bayati \emph{et. al} \cite{Mohsen15} and Chen \emph{et. al} \cite{chen2020}, right-orthogonally-invariant $\bA$ by Rangan \emph{et. al} \cite{Rangan2019}, rotationally-invariant $\bA$\footnote{A matrix $\bA$ is said  rotationally-invariant if $P(\bA) = P(\bU \bA \bV)$ for any deterministic orthogonal matrices $\bU$ and  $\bV$, where $P(\bA)$ is the probability distribution function of a matrix $\bA$ and a matrix is said orthogonal if its columns (rows) are orthogonal vectors.} by Fan \cite{Zhou2020}, and unitarily-invariant $\bA$\footnote{The matrix $\bA = \bU\Sigma\bV^T$ is said unitarily-invariant if $\bU$, $\bV$, and $\Sigma$ are mutually independent, and $\bU$, $\bV$ are isotropically distributed in the space of unitary matrices, which is the set of square complex matrices with orthonormal columns (rows).} by Takeuchi \cite{Takeuchi2020}.
    %%
    The results in \cite{Zhou2020} contain those in \cite{Rangan2019}. The results in \cite{Takeuchi2020} is an extension of \cite{Rangan2019} to the complex $\bA$. 
    %%
    Understanding the dynamics of AMP for a range of measurement ensembles \cite{Mohsen15, chen2020, Takeuchi2020, Rangan2019, Zhou2020} was a significant progress.
    %%
    A belief is that the SE for AMP might hold for an even boarder class of matrices.  
    %%
    %%
    \begin{figure}[htp]
  	\centering
 	\includegraphics[width=0.5\textwidth]{VenDiagram.pdf} %\vspace* {-0.7cm}
 	\caption{Two categories of random matrices}
    	\label{Fig1}
 	 \vspace*{-0.4cm}
    \end{figure} 
    %%
    
    %%
   The key to analyzing the SE for AMP is the conditioning technique \cite{Bolthausen2009, Bayati11}, identifying the distribution of $\bA$ at the $t$th iteration conditioned on the last $(t-1)$ iterations of the AMP algorithm.
   %% 
   This means that the $t$th iteration of the AMP algorithm is modeled as a linear combination of the previous $(t-1)$ iterations instances, a Gaussian random variable, plus a deviation term. 
   %%
   A key step to the stability proof of AMP is leveraging the polynomial smoothness of the pseudo-Lipschitz function\footnote{For a $k > 1$, a function $f:\R^{n \times 1} \rightarrow \R$ is said pseudo-Lipschitz of order $k$ if there exists a constant $L > 0$ such that $|f(\bx)-f(\by)| \leq L(1+\|\bx\|^{k-1}+\|\by\|^{k-1})\|\bx-\by\|$, for all $\bx, \by \in \R^{n \times 1}$. The first order derivative of $f$ is bounded by a polynomial of order $(k-1)$, i.e., polynomial smoothness.} and establishing that the contribution of the deviation term to the instantaneous distribution falls in $n$ and $N$.   
   %%
    
    %%
    Recently, the class of controlled function, which will be defined in Section~\ref{Sec:Assumption} and will be incorporated in our derivation, has been introduced to model the nonlinear behavior of neural networks in machine learning \cite{yangTP1,yang2019}.
    %% 
    %%
    Unlike the pseudo-Lipschitz function that has polynomial growth, the controlled function can increase exponentially; it is still measurable against Gaussian measure in $\cL^1$ and $\cL^2$ space \cite{yangTP1,yang2019}. 
    %%
    Hence, the pseudo-Lipschitz function is a special case of the controlled function.
    %%
    \subsection{Overview of Contributions}\label{contributions}
    %%
    This work is motivated by the observation that the dynamic of AMP is induced in the structure of the random measurement ensemble and the class of functions assumed to characterize SE. 
    %%
    The major contributions are summarized below. 
    %%
    \begin{itemize}
    \item 
    %%
    The class of random measurement matrices in this work distinguishes it from the one in prior works \cite{Takeuchi2020,Rangan2019,Zhou2020} which corresponds to $\cR$ in Fig.~\ref{Fig1}, where $\cR$ denotes the set of rotationally-invariant matrices.
    %%
    Specifically, we extend the SE analysis for AMP to measurement ensemble $\bA \in \cI$ in Fig.~\ref{Fig1} where $\cI$ is the set of matrices with independent but  not necessarily identically distributed entries, which includes the  i.i.d. Gaussian $\bA$ \cite{Bayati11,Rush2018} (i.e., $\bA \in \cI \cap \cR$ in Fig.~\ref{Fig1}). 
    %%
    Our result is a theoretical justification for the conjecture made in \cite{Bayati11} about the validity of the SE for AMP with i.i.d. non-Gaussian measurement ensembles. 
    %%
    %% 
    Although a similar SE analysis framework to \cite{Bayati11} is adopted in this work, our solution approach reveals a new direction to deal with the set $\cI$. 
    %% 
    We present a mathematical treatment to characterize an asymptotic behavior of AMP with the measurement matrices in $\cI$. 
    %%
    The lack of structure of the matrices in $\cI$ is addressed by extending the Linderberg-Feller theorem to the set $\cI$.
    %%
    This development provides a useful basis for establishing the SE with the set $\cI$. 
    \item 
    In contrast with prior works \cite{Bayati11,Mohsen15,chen2020,Ma2017,Takeuchi2020,Rangan2019,Zhou2020} that established the SE with the pseudo-Lipschitz function, we generalize the proof of SE to the class of controlled functions. 
    %%
    An empirical statistic-based conditioning technique is proposed to cope with the lack of polynomial smoothness of the controlled function.
    %%
    While the previous works established SE by utilizing the polynomial growth of the pseudo-Lipschitz function, this work exploits the measurability of the controlled function to deal with its exponential growth.  
    %%
    \end{itemize}
    
    %%
    \textit{Notation}: A lowercase letter in bold $\ba$ is a column vector and a uppercase letter in bold $\bA$ is a matrix.
    %%
    $\|\ba\|_p$, $\bA^*$, and $A_{ij}$ denote the $p$-norm of $\ba$, transpose of $\bA$, and $i$th row and $j$th column entry of $\bA$, respectively. 
    %%  
    $\bA(N)$ and $\ba(N)$ mean that the matrix and vector are indexed by $N$.   
    %%
    $\cN(\nu,\sigma^2)$ denotes the Gaussian distribution with mean $\nu$ and variance $\sigma^2$.
    %%
    The $\xRightarrow{d}$ and $\das$ denote the convergence in distribution and equivalence in an almost sure sense, respectively.
    %%
    $\lL\bu,\bv \lR = \frac{1}{n}\sumn u_iv_i$ defines the normalized scalar product of  $\bu, \bv \in \R^{n \times 1}$.
    %%
    $\E[\cdot]$ and $\E_{Z}[\cdot]$ denote the expectation and the expectation with respect to the random variable $Z$, respectively.  
    %%
%%

==> Proof.tex <==
\section{Proof of Theorem 1}
\label{secIV}

 The proof of {Theorem}~\ref{theorem1} is conducted by induction with respect to $t$, which consists of four steps corresponding to applying conditioning technique on four sets $\cF_{0,0}$, $\cF_{1,0}$, $\cF_{t,t}$, and $\cF_{t+1,t}$, respectively.
 %%
 The following proof is inspired by the  framework in \cite[Lemma~1]{Bayati11} and refined for the class of random measurement matrix $\bA$ defined as in Section~\ref{Sec:Assumption} and the controlled functions defined in \eqref{eq:controlled1}. 
%%
Noting that sending $n$ or $N$ to infinity has the same meaning because $\rho = \frac{n}{N}$ is always kept constant.
%%
In what follows, all convergence results are obtained when either $n$ or $N$ tends to infinity unless specified otherwise.
%%
%%
\subsection{Step 1: Conditioning on $\cF_{0,0} = \{\bq^0,\bx_0,\bw\}.$}
%%
\noindent a) 
 The \eqref{eq:b1} is straightforward when $t=0$ because $\bb^0 = \bA\bq^0$ and $\bq^{0}_{\perp} = \bq^0$. \\
%%
b) The \eqref{eq:alphaQ} is straightforward due to the fact that $\bq^{0}_{\perp} = \bq^0$ and the assumption of $\bq^0$ in the definition of SE in \eqref{eq:SE}.\\
%%
c)
%%
 We have the assumptions $\limN \frac{\lL\bq^0,\bq^0 \lR}{\rho} =  \sigma^2_0$ and $\limsupN \frac{1}{N}\sumN |q^0_i|^{2+2\alpha} < \infty $ for a constant $\alpha > 1$.
 %%
 Hence, applying {Proposition}~\ref{ps6} to $\bA$ and $\bq^0$ leads to the convergence,  
 \begin{equation}
     \label{eq:1.1}
     \widehat{\bA \bq^0} \xRightarrow{d} \cN(0,\sigma^2_0).
 \end{equation}
 Hence, $\widehat{\bb^0} \xRightarrow{d} \cN(0,\sigma^2_0)$, implying  $\limn \lL \bb^0, \bb^0\lR \das \sigma^2_0.$
Thus, $\limn \lL \bb^0, \bb^0 \lR \das \limN \frac{\lL \bq^0,\bq^0\lR}{\rho} < \infty$, which completes the proof of \eqref{eq:b2} when $t=0$. \\
%%
d) We let $\widetilde{\bu}^0_i=(\sigma_0 \widetilde{Z}_0,w_i)$, for $i =1,2,\dots,n$, where $\widetilde{Z}_0 \sim \cN(0,1)$.
%%
By the result in \eqref{eq:1.1}, the convergence  $\bu^0_i= (b^0_i,w_i) \xRightarrow{d}  \widetilde{\bu}^0_i$ holds, for $i =1,2,\dots,n$.
%%
To prove \eqref{b:b}, it is needed to show that 
$\limn \frac{1}{n}\sumn \phi_b(\widetilde{\bu}^0_i) \das \E[\phi_b(\sigma_0\widetilde{Z}_0,W)]$.
%, i.e.,  $\limn \frac{1}{n}\sumn \phi_b(\widetilde{\bu}^0_i) - \E[\phi_b(\sigma_0\widetilde{Z}_0,W)]\das 0$.
%%
Now, using the triangular inequality we have
\begin{equation}
    \label{eq:1.3}
    \bigg|\frac{1}{n}\sumn \phi_b(\widetilde{\bu}^0_i) - \E[\phi_b(\sigma_0\widetilde{Z}_0,W)]\bigg| \leq X^0_1 + X^0_2,
\end{equation}
 where $X^0_1 = \bigg|\frac{1}{n}\sumn \bigg(\phi_b(\widetilde{\bu}^0_i) - \E_{\widetilde{Z}_0}[\phi_b(\widetilde{\bu}^0_i)]\bigg) \bigg|$ and $X^0_2 = \bigg|\frac{1}{n}\sumn \E_{\widetilde{Z}_0}[\phi_b(\widetilde{\bu}^0_i)] - \E[\phi_b(\sigma_0\widetilde{Z}_0,W)] \bigg|$. 
 %%
 In what follows, we are going to verify that $\limn X^0_1 \das 0$ and $\limn X^0_2 \das 0$, respectively. 
%%

%%
Since $\phi_b$ is a controlled function defined in \eqref{eq:controlled1}, the following holds  $|\phi_b(\widetilde{\bu}^0_i)| \leq c^0_1 \exp(c^0_2(|\sigma_0\widetilde{Z}_0|^{\lambda} + |w_i|^{\lambda}))$ due to \eqref{eq:controlled2}, where $0 < c^0_1$, $0 < c^0_2$, and $1 < \lambda <2$ are constants. 
%%
Hence, $\E_{\widetilde{Z}_0}[|\phi_b(\widetilde{\bu}^0_i)|^{2+\kappa}] \leq c^0_3 \exp(c^0_4|w_i|^{\lambda}) \E_{\widetilde{Z}_0}[\exp(c^0_4|\sigma_0\widetilde{Z}_0|^{\lambda})],$ where $0<\kappa <1$, $c^0_3 = (c^0_1)^{2+\kappa}$, and $c^0_4 = c^0_2(2+\kappa)$.
%%
Thus, 
\begin{equation}
    \label{eq:1.2}
    \E_{\widetilde{Z}_0}[|\phi_b(\widetilde{\bu}^0_i)|^{2+\kappa}] \leq c^0_5 \exp(c^0_4|w_i|^{\lambda}),
\end{equation}
where $c^0_5 = c^0_3 \E_{\widetilde{Z}_0}[\exp(c^0_4|\sigma_0\widetilde{Z}_0|^{\lambda})]$ is a constant.
%%
We define $X_{n,i} = \phi_b(\widetilde{\bu}^0_i) - \E_{\widetilde{Z}_0}[\phi_b(\widetilde{\bu}^0_i)]$, for $i =1,2,\dots,n$. 
%%
To verify the convergence $\limn X^0_1 \das0$, we will show that $\{X_{n,i}\}^n_{i=1}$ satisfy the condition of {Lemma}~\ref{lm3}.
%%
Indeed, applying {Lemma}~\ref{lm4} to $X_{n,i}$ $=$ $\phi_b(\widetilde{\bu}^0_i) - \E_{\widetilde{Z}_0}[\phi_b(\widetilde{\bu}^0_i)]$ gives 
\begin{subequations}
\label{eq:1.3.1}
\beq 
\E_{\widetilde{Z}_0}[|X_{n,i}|^{2+\kappa}] &\leq& 2^{1+\kappa}\bigg[\E_{\widetilde{Z}_0}[|\phi_b(\widetilde{\bu}^0_i)|^{2+\kappa}]  +  \bigg|\E_{\widetilde{Z}_0}[\phi_b(\widetilde{\bu}^0_i)]\bigg|^{2+\kappa} \bigg], \nonumber\\ 
&\leq& 2^{1+\kappa}\bigg[\E_{\widetilde{Z}_0}[|\phi_b(\widetilde{\bu}^0_i)|^{2+\kappa}]  +  \E_{\widetilde{Z}_0}[|\phi_b(\widetilde{\bu}^0_i)|^{2+\kappa}] \bigg],\label{eq:1.3c}\\
&\leq& c^0_6\exp(c^0_4|w_i|^{\lambda}),\label{eq:1.3e} 
\eeq 
\end{subequations}
where \eqref{eq:1.3c} follows from {Lemma}~\ref{lm5} and \eqref{eq:1.3e} is due to \eqref{eq:1.2} with $c^0_6 = 2^{2+\kappa}c^0_5$. Therefore,    
\begin{equation}
  \frac{1}{n}\sumn \E_{\widetilde{Z}_0}[|X_{n,i}|^{2+\kappa}] \leq \frac{1}{n} \sumn c^0_6\exp(c^0_4|w_i|^{\lambda})  
  \das \E[c^0_6\exp(c^0_4|W|^{\lambda})] < cn^{\kappa/2},\label{eq:1.4b}  
\end{equation} for $n$ is sufficient large, where $c$ is a positive constant and the last estimation in \eqref{eq:1.4b} follows from the facts that $\E[c^0_6\exp(c^0_4|W|^{\lambda})]=c^0_7< \infty$ and $c_7 < cn^{\kappa}$ as $n_0<n$, for a constant $n_0$.
%%
Given \eqref{eq:1.4b}, applying {Lemma}~\ref{lm3} leads to $\limn \frac{1}{n}\sumn X_{n,i} \das 0$, implying $\limn X^0_1 \das 0$.   
%%

%%
 The rest of part d) in {Step}~1 is showing the convergence $\limn X^0_2 \das0$. We define $\widetilde{\phi}_b(w_i) = \E_{\widetilde{Z}_0}[\phi_b(\widetilde{\bu}^0_i)]$, for $i =1,2,\dots,n$.  
 %%
 Then $\limn \frac{1}{n}\sumn \widetilde{\phi}_b(w_i) \das \E[\widetilde{\phi}_b(W)]$ since $\widehat{\bw} \xRightarrow{d} \mu_W$. 
 %%
 Hence, $\limn \frac{1}{n} \sumn \E_{\widetilde{Z}_0}[\phi_b(\widetilde{\bu}^0_i)] \das \E[\E_{\widetilde{Z}_0}[\phi_b(\sigma_0\widetilde{Z}_0,W)]] = \E[\phi_b(\sigma_0\widetilde{Z}_0,W)]$,
which leads to $\limn X^0_2 \das 0$.
%%
Therefore, substituting $\limn X^0_1 \das 0$ and $\limn X^0_2 \das 0$ into \eqref{eq:1.3} gives $\limn \frac{1}{n}\sumn \phi_b(\widetilde{\bu}^0_i) - \E[\phi_b(\sigma_0\widetilde{Z}_0,W)] \das 0$, which completes the proof of \eqref{b:b} when $t=0$.     
 \subsection{Step 2: Conditioning on $\cF_{1,0} = \{\bb^0,\bm^0,\bq^0,\bx_0,\bw\}.$}
a) From the general AMP recursion in \eqref{eq:6}, $\bh^1|_{\cF_{1,0}} \ddis \bA^*|_{\cF_{1,0}}\bm^0 - \xi_0\bq^{0}$.
%%
Note that conditioning on $\cF_{1,0}$ is equivalent to conditioning on the set $\{\bA |\bA\bq^0=\bb^0 \}$. 
Hence, applying {Proposition}~\ref{ps4} yields   $\bA|_{\cF_{1,0}} \ddis \widetilde{\bA}\bP^{\perp}_{\bq^{0}} +\bb^0\frac{1}{\|\bq^0\|^2_2}{\bq^{0}}^*$.
%%
Then $\bh^1|_{\cF_{1,0}}$ follows  
\begin{equation}
    \bh^1|_{\cF_{1,0}} \ddis \bP^{\perp}_{\bq^0}\widetilde{\bA}^*\bm^0 + \frac{{\bb^{0}}^*\bm^0}{\|\bq^0\|^2_2}\bq^0 - \xi_0\bq^0 =  {\widetilde{\bA}}^*\bm^0-\bP_{\bq^0} {\widetilde{\bA}}^*\bm^0 +\bigg(\rho \frac{\lL\bb^0,\bm^0\lR}{\lL\bq^0,\bq^0\lR}-\xi_0\bigg)\bq^0. \label{eq:2.1}
\end{equation}
In \eqref{eq:2.1}, substituting $\bm^0 = g_0(\bb^0,\bw)$ into the term $\lL \bb^0,\bm^0 \lR$ gives the convergence,  
\begin{subequations}
\label{eq:2.2}
\beq 
 \limn \lL \bb^0,\bm^0 \lR = \limn \lL \bb^0, g_0(\bb^0,\bw) \lR &\das& \E[\sigma_0 \widetilde{Z}_0g_0(\sigma_0 \widetilde{Z}_0,W)],\label{eq:2.2a}\\ 
    &\das& \sigma^2_0 \E[g'_0(\sigma_0\widetilde{Z},W)],\label{eq:2.2b}\\
    &\das& \limn \lL \bb^0,\bb^0\lR \lL g_0'(\bb^0,\bw) \lR,\label{eq:2.2c}\\
    &\das& \limN \frac{\lL\bq^0,\bq^0 \lR}{\rho}\xi_0, \label{eq:2.2d}
\eeq 
\end{subequations} 
%%
where \eqref{eq:2.2a} is a result of applying \eqref{b:b} to $\phi_b(\bu^0_i) = b^0_ig_0(b^0_i,w_i)$ at $t=0$, \eqref{eq:2.2b} is due to {Lemma}~\ref{lm2}, \eqref{eq:2.2c} is obtained by setting $\phi_b(\bu^0_i) = g'_0(b^0_i,w_i)$ in \eqref{b:b} at $t= 0$, and \eqref{eq:2.2d} follows from the fact that $\xi_0 = \lL g'_0(\bb^0,\bw)\lR$ and using \eqref{eq:b2} with $t_1=t_2=0$. 
%%
Substituting \eqref{eq:2.2d} into   \eqref{eq:2.1} leads to
    \begin{equation}
        \label{eq:2.3}
        \bh^1|_{\cF_{1,0}} \ddis  \widetilde{\bA}^*\bm^0-\bP_{\bq^0} \widetilde{\bA}^*\bm^0 +o(1)\bq^0,
    \end{equation} where $\limn o(1) \das 0$. Using {Proposition}~\ref{ps3}, the second term in the right-hand side of \eqref{eq:2.3} converges to $\limN \bP_{\bq^0} \widetilde{\bA}^*\bm^0 \das \mathbf{0}_N$. 
    %%
    Similarly, the last term converges to $\limN o(1)\bq^0 \das \mathbf{0}_N$. Indeed, the empirical expectation of $o(1)\bq^0$ satisfies $\limN \lL \widehat{o(1)\bq^0} \lR \das 0$, which holds because  $\limN |\lL\widehat{o(1)\bq^0}\lR| \leq \limN |o(1)| \frac{1}{N}\sumN |q^0_i| \das 0$, and the empirical variance of $o(1)\bq^0$ converges to $\limN \lL \widehat{o(1)\bq^0} \lR_2 = \limN [o(1)]^2\lL\bq^0,\bq^0 \lR \das 0$ because $\limN \lL\bq^0,\bq^0 \lR < \infty$. 
    %%
    Thus,  $\bh^1|_{\cF_{1,0}} \xRightarrow{d} \widetilde{\bA}^*\bm^0$, which concludes \eqref{eq:h1} when $t = 0$ since $\bm^0 = \bm^0_{\perp}$.\\ 
    b) The \eqref{eq:alphaM} is equivalent to $\limsupn \frac{1}{n} \sumn |m^0_i|^{2+2\alpha} < \infty$, which holds because substituting $\phi_b(b^0_i,w_i) = [g_0(b^0_i,w_i)]^{1+\alpha}$ to \eqref{b:b} at $t=0$ leads to $\limn \lL g^{1+\alpha}_0(\bb^0,\bw),g^{1+\alpha}_0(\bb^0,\bw)\lR\das \E[g^{2+2\alpha}_0(\sigma_0\widetilde{Z}_0,W)]$. Hence, $\limn \frac{1}{n} \sumn |m^0_i|^{2+2\alpha} \das \E[g^{2+2\alpha}_0(\sigma_0\widetilde{Z}_0,W)] < \infty$, which completes the solution of \eqref{eq:alphaM} at $t=0$.\\
    c) Setting $\phi_b(b^0_i,w_i) = g_0(b^0_i,w_i)$ in \eqref{b:b} at $t=0$, we get  $\limn \lL g_0(\bb^0,\bw),g_0(\bb^0,\bw)\lR\das \E[g^2_0(\sigma_0\widetilde{Z}_0,W)]$. 
    %%
    Thus, the following holds due to the definitions of $\bm^0$ in \eqref{eq:6} and $\tau^2_0$ in \eqref{eq:SE}, $\limn \lL\bm^0,\bm^0 \lR \das \tau^2_0$.
    %%
    We now note that $\bm^0_{\perp} = \bm^0$ satisfies the condition in {Proposition}~\ref{ps6} due to \eqref{eq:alphaM} when $t=0$.
    %%
    Hence, using {Proposition}~\ref{ps6} for $\widetilde{\bA}^*$ and $\bm^0$ leads to the convergence  $\widehat{\widetilde{\bA}^*\bm^0} \xRightarrow{d} \cN(0,\tau^2_0)$, implying $\widehat{\bh^1} \xRightarrow{d} \cN(0,\tau^2_0)$, i.e., $\limN \lL\bh^1,\bh^1\lR \das \tau^2_0$. Hence, $\limN \lL\bh^1,\bh^1\lR \das \limn \lL\bm^0,\bm^0 \lR < \infty$, which concludes \eqref{eq:h2} when $t= 0$.\\
    d) We define $\widetilde{\bv}^0_i=(\tau_0Z_0,x_{0i})$, for $i =1,2,\dots, N$. 
    %%
    The convergence $\bv^0_i = (h^1_i,x_{0i}) \xRightarrow{d} \widetilde{\bv}^0_i$ holds because $\widehat{\bh^1} \xRightarrow{d} \cN(0,\tau^2_0)$, for $i =1,2,\dots, N$. 
    %%
    To prove \eqref{b:h}, it is needed to show that $\limN \frac{1}{N}\sumN \phi_h(\widetilde{\bv}^0_i) \das \E[\phi_h(\tau_0Z_0,X_0)]$. 
    %%
    Similar to part d) of {Step} 1, following from the triangular inequality, we will claim that $\limN Y^0_1 \das 0$ and $\limN Y^0_2 \das 0$, where $Y^0_1 = \bigg|\frac{1}{N}\sumN \left(\phi_h(\widetilde{\bv}^0_i) - \E_{Z_0}[\phi_h(\widetilde{\bv}^0_i)]\right)\bigg|$ and  $Y^0_2 = \bigg|\frac{1}{N} \sumN \E_{Z_0}[\phi_h(\widetilde{\bv}^0_i)] - \E[\phi_h(\tau_0Z_0,X_0)]\bigg|$.
    %%
    
    %%
    We first define $Y_{N,i} = \phi_h(\widetilde{\bv}^0_i) - \E_{Z_0}[\phi_h(\widetilde{\bv}^0_i)],$ for $i = 1,2,\dots,N$.
    %%
    To verify the convergence $\limN Y^0_1 \das 0$, we will show that $\{Y_{N,i}\}_{i=1}^{N}$ satisfy the condition of {Lemma}~\ref{lm3}.
    %%
    Since $\phi_h$ is a controlled function, the following holds $|\phi_h(\widetilde{\bv}^0_i)| \leq d^0_1 \exp(d^0_2(|\tau_0Z_0|^{\lambda} + |x_{0i}|^{\lambda}))$ due to \eqref{eq:controlled2}, where $0 < d^0_1$, $0 < d^0_2$, and $1 \leq  \lambda < 2$ are constants.
    %%
    Hence, $\E_{Z_0}[|\phi_h(\widetilde{\bv}^0_i)|^{2+\kappa}] \leq d^0_3\exp(d^0_4|x_{0i}|^{\lambda})\E_{Z_0}[\exp(d^0_4|\tau_0Z_0|^{\lambda})]$, where $0 < \kappa < 1$, $d^0_3 = (d^0_1)^{2+\kappa},$ and $d^0_4 = d^0_2(2+\kappa)$.
    %%
    Therefore, 
    \begin{equation}
    \label{eq:2.4}
    \E_{Z_0}[|\phi_h(\widetilde{\bv}^0_i)|^{2+\kappa}] \leq d^0_5\exp(d^0_4|x_{0i}|^{\lambda}),
    \end{equation}
    where $d^0_5 = d^0_3\E_{Z_0}[\exp(d^0_4|\tau_0Z_0|^{\lambda})]$ is a constant. Applying {Lemma} 4 to $Y_{N,i} = \phi_h(\widetilde{\bv}^0_i) - \E_{Z_0}[\phi_h(\widetilde{\bv}^0_i)]$ yields
    \begin{subequations}
    \label{eq:2.5}
    \beq 
        \E_{Z_0}[|Y_{N,i}|^{2+\kappa}] &\leq& 2^{1+\kappa}\bigg[\E_{Z_0}[|\phi_h(\widetilde{\bv}^0_i)|^{2+\kappa}] + \bigg|  \E_{Z_0}[\phi_h(\widetilde{\bv}^0_i)]\bigg|^{2+\kappa} \bigg],\nonumber\\
        &\leq& 2^{1+\kappa}\bigg[\E_{Z_0}[|\phi_h(\widetilde{\bv}^0_i)|^{2+\kappa}] + \E_{Z_0}[|\phi_h(\widetilde{\bv}^0_i)|^{2+\kappa}] \bigg],\label{eq:2.5c}\\ 
        &\leq& d^0_6 \exp(d^0_4|x_{0i}|^{\lambda})\label{eq:2.5e},
    \eeq
    \end{subequations} where \eqref{eq:2.5c} follows from Lemma~\ref{lm5} and \eqref{eq:2.5e} is due to \eqref{eq:2.4} with $d^0_6 =2^{2+\kappa}d^0_5$.
    %%
    Therefore, 
    \begin{equation}
        \frac{1}{N}\sumN \E_{Z_0}[|Y_{N,i}|^{2+\kappa}] \leq \frac{1}{N}\sumN d^0_6 \exp(d^0_4|x_{0i}|^{\lambda}) \das \E[d^0_6\exp(d^0_4|X_0|^{\lambda})]<  cN^{\kappa/2}, \label{eq:2.6c}
    \end{equation}
    for $N$ is sufficiently large, 
    where $c$ is a possitive constant and the last estimation in \eqref{eq:2.6c} follows from the facts that $\E[d^0_6\exp(d^0_4|X_0|^{\lambda})] = d^0_7 < \infty$ and $d^0_7 < cN^{\kappa/2}$ as $N_0 < N$, for a constant $N_0$.
    %%
    Given \eqref{eq:2.6c}, applying {Lemma}~\ref{lm3} to $\{Y_{N,i}\}_{i=1}^{N}$ gives $\limN \frac{1}{N}\sumN Y_{N,i} \das 0$, implying $\limN Y^0_1 \das 0$. 
    %%
    
    %%
    To show $\limN Y^0_{2}\das 0$, we define $\widetilde{\phi}_h(x_{0i}) = \E_{Z_0}[\phi_h(\widetilde{\bv}^0_i)]$. 
    %%
    Then the following convergence holds,
    $\limN \frac{1}{N} \sumN \widetilde{\phi}_h(x_{0i}) \das \E[\widetilde{\phi}_h(X_0)]$ due to the fact that $\widehat{\bx_0} \xRightarrow{d} \mu_{X_0}$.
    %%
    Therefore, $\limN \frac{1}{N} \sumN \E_{Z_0}[\phi_h(\widetilde{\bv}^0_i)] \das \E[\E_{Z_0}[\phi_h(\tau_0Z_0,X_0)]]=\E[\phi_h(\tau_0Z_0,X_0)]]$, which leads to $\limN Y^0_2 \das 0$. 
    %%
    Hence, we have verified our claim at the beginning of part d) in {Step} 2, which completes the proof of \eqref{b:h} when $t=0$.   
    %%

    %%
    Assume that {Theorem}~\ref{theorem1} holds up to the $(t-1)$th iteration. 
    %%
    We will prove it also holds for the $t$th iteration.
    %%
    In what follows, we will show \eqref{eq:b1}, \eqref{eq:alphaQ}, \eqref{eq:b2}, and \eqref{b:b} in {Step}~3 and \eqref{eq:h1}, \eqref{eq:alphaM}, \eqref{eq:h2},  and \eqref{b:h} in {Step}~4, respectively. 
    
    \subsection{Step 3: Conditioning on $\cF_{t,t} = \{\bb^0,\dots,\bb^{t-1},\bm^0,\dots,\bm^{t-1},\bh^1,\dots,\bh^t,\bq^0,\dots,\bq^t,\bx_0,\bw\}$.}
    a)
    %%
    Noting that conditioning on $\cF_{t,t}$ is equivalent to conditioning on $\cP_{\bX_t,\bY_t} = \{\bA|\bA^*\bM_t = \bX_t, \bA\bQ_t = \bY_t\}$. 
    %%
    Hence, applying Proposition~\ref{ps4} to obtain the conditional distribution 
    $\bA|_{\cF_{t,t}}$ and following the same procedure as in \cite[Lemma 1a]{Bayati11}, the conditional distribution of $\bb^t$ on $\cF_{t,t}$ is given by 
    \begin{equation}
    \label{eq:3.1}
        \bb^t|_{\cF_{t,t}} \ddis  \sum_{j=0}^{t-1}\beta_j\mathbf{b}^j + \widetilde{\bA}\bq^{t}_{\perp} - \bP_{\bM_t}\widetilde{\bA}\bq^t_{\perp}+ \mathbf{M}_t\overrightarrow{\bo_t}(1).
    \end{equation}
    %%
    By {Proposition}~\ref{ps3}, the third term in the right-hand side of \eqref{eq:3.1} converges to $\limn \bP_{\bM_t}\widetilde{\bA}\bq^t_{\perp} \das \mathbf{0}_n$.
    %%
    Similar to part a) of {Step}~2, we verify the convergence $\limn \bM_t\overrightarrow{\bo}_t(1)\das \mathbf{0}_n$ by characterizing the expectation and variance of its empirical distribution $\widehat{\bM_t\overrightarrow{\bo}_t(1)}$ as $n \rightarrow \infty$.
    %%
    Indeed,  
    \begin{equation}
    \label{eq:3.2}
            \limn |\lL \bM_t\overrightarrow{\bo}_t(1) \lR| \leq \limn |o(1)|\frac{1}{n}\sum_{i=1}^{n}\bigg|\sum_{j=0}^{t-1}m^j_i\bigg| \leq \limn |o(1)|\sum_{j=0}^{t-1}\frac{1}{n}\sum_{i=1}^{n}|m^j_i| \das  0,
    \end{equation}
    where the last equality in \eqref{eq:3.2} holds because applying $\phi_b (b^j_i,w_i) = g_j(b^j_i,w_i)$ to the induction hypothesis in \eqref{b:b}, $\forall j < t,$ leads to $\limn \frac{1}{n}\sum_{i=1}^{n}|m^j_i| \das \E[|g_j(\sigma_j\widetilde{Z}_j,W)|] < \infty$.  
    %%
    Hence, $\limn \lL \bM_t\overrightarrow{\bo}_t(1) \lR \das 0$. The variance of $\widehat{\bM_t\overrightarrow{\bo}_t(1)}$ converges to 
    \begin{subequations}
    \label{eq:3.3}
    \beq
    \limn \lL \bM_t \overrightarrow{\bo}_t(1) \lR_2 = \limn \frac{1}{n}[o(1)]^2 \sum_{i=1}^{n}\bigg( \sum_{j=0}^{t-1}m^j_i \bigg)^2  
    &\leq& \limn [o(1)]^2 t \frac{1}{n}\sum_{i=1}^{n} \sum_{j=0}^{t-1}(m^j_i)^2, \label{eq:3.3a}\\
    & = & \limn [o(1)]^2t\sum_{j=0}^{t-1}\lL\bm^j,\bm^j\lR \das 0, \label{eq:3.3b}
    \eeq
    \end{subequations}
    where \eqref{eq:3.3a} follows from the Cauchy-Schwarz inequality and \eqref{eq:3.3b} holds because applying induction hypothesis for $\phi_b(b^j_i,w_i) = g^2_j(b^j_i,w_i)$ in \eqref{b:b} gives $\limn \lL\bm^j,\bm^j \lR \das \E[g^2_j(\sigma_j\widetilde{Z}_j,W)] < \infty$, for $j =0,1,\dots, t-1$.
    %%
    Hence, \eqref{eq:3.3b} is equivalent to $\limn \lL \bM_t \overrightarrow{\bo}_t(1) \lR_2 \das 0$. 
    %%
    Therefore, $\limn \bM_t \overrightarrow{\bo}_t(1) \das \mathbf{0}_n$, implying 
    \begin{equation}
        \label{eq:3.4}
        \bb^t|_{\cF_{t,t}} \xRightarrow{d} \sum_{j=0}^{t-1}\beta_j\bb^j + \widetilde{\bA}\bq^t_{\perp},
    \end{equation}
     which completes the proof of \eqref{eq:b1} at the $t$th iteration.\\
    %%
    b) Applying \eqref{b:h} to $\phi_h(h^t_i,x_{0i}) = f^{1+\alpha}_t(h^t_i,x_{0i})$ yields $\limN \frac{1}{N} \sumN |q^t_i|^{2+2\alpha} \das \E[f^{2+2\alpha}_t(\tau_{t-1}Z_{t-1},X_0)] < \infty.$ Because $\sumN |q^t_{\perp i}|^{2+2\alpha} < \sumN |q^t_{i}|^{2+2\alpha}$, the following holds,    
    $\limsupN \frac{1}{N} \sumN |q^t_{\perp i}|^{2+2\alpha} < \infty$, which concludes \eqref{eq:alphaQ} at the $t$th iteration.\\
    %%
    c) For $t_1 < t$ and $t_2=t$, the convergence $\limn \lL \bb^{t_1},\bb^{t} \lR$ is given by
    \begin{subequations}
    %\label{eq:3.5}
    \beq
     \limn \lL\bb^{t_1},\bb^t\lR &\ddis& \limn \sum_{j=0}^{t-1} \beta_j\lL\bb^{t_1},\bb^j\lR +\limn  \lL \bb^{t_1},\widetilde{\bA}\bq^t_{\perp}\lR, \label{eq:3.5a}\\
    &\das&  \sum_{j=0}^{t-1} \beta_j\limN\frac{\lL\bq^{t_1},\bq^j\lR}{\rho} + \limn \frac{\bb^{t_1^*}\widetilde{\bA}\bq^t_{\perp}}{n} \label{eq:3.5b}, 
    \eeq
    \end{subequations} where \eqref{eq:3.5a} follows from \eqref{eq:3.4} and \eqref{eq:3.5b} is a result of applying the induction hypothesis to \eqref{eq:b2} for $t_1 < t$ and $t_2 = j < t$. 
    %%
    We will show that the second term in \eqref{eq:3.5a} converges to $0$ almost surely. Applying {Proposition}~\ref{ps7} gives $ \frac{\bb^{t_1^*}}{\|\bb^{t_1}\|_2}\widetilde{\bA}\frac{\bq^t_{\perp}}{\|\bq^t_{\perp}\|_2} \ddis \frac{Z}{\sqrt{n}}$, where $Z \sim \cN(0,1)$. Hence, 
    %%
    \begin{equation}
\frac{\bb^{t_1^*}\widetilde{\bA}\bq^t_{\perp}}{n} \ddis  \frac{\|\bb^{t_1}\|_2}{\sqrt{n}}\frac{\|\bq^t_{\perp}\|_2}{\sqrt{N}}\frac{1}{\sqrt{\rho}}\frac{Z}{\sqrt{n}}
    =\frac{1}{\sqrt{\rho}} \sqrt{\lL\bb^{t_1},\bb^{t_1} \lR \lL\bq^t_{\perp},\bq^t_{\perp}\lR} \frac{Z}{\sqrt{n}}.\label{eq:3.6}
    \end{equation}
    In \eqref{eq:3.6}, the $\lL\bb^{t_1},\bb^{t_1} \lR$ converges to $\limn \lL\bb^{t_1},\bb^{t_1} \lR = \limn \frac{\lL \bq^{t_1},\bq^{t_1} \lR}{\rho} < \infty$, which follows  from the induction hypothesis in \eqref{eq:b2} at $t_1 < t$ and the $\lL\bq^t_{\perp},\bq^t_{\perp}\lR$ converges to $\limN \lL\bq^t_{\perp},\bq^t_{\perp}\lR < \limN \lL\bq^t,\bq^t\lR < \infty$. 
    %%
    The last estimation follows because $q^t_i= f^2_t(h^t_i,x_{0i})$ and applying \eqref{b:h} for $\phi_h(h^t_i,x_{0i}) = f^2_t(h^t_i,x_{0i})$ yields $\limN \lL\bq^t,\bq^t\lR  = \frac{1}{N}\sumN f^2_t(h^t_i,x_{0i}) \das \E[f^2_t(\tau_{t-1}Z_{t-1},X_0)] < \infty$. 
    %%
    Thus, 
    \begin{equation}
        \label{eq:3.7}
      \limn  \lL\widetilde{\bA}\bq^t_{\perp},\bb^{t_1}\lR = \limn \frac{\bb^{t_1^*}\widetilde{\bA}\bq^t_{\perp}}{n} \das 0, \text{ for } t_1 < t. 
    \end{equation} Substituting \eqref{eq:3.7} into \eqref{eq:3.5a} gives  
    \begin{subequations}
    \label{eq:3.8}
    \beq 
    \d4 \d4 \d4\d4 \d4\d4 \limn \lL\bb^{t_1},\bb^t\lR \das  \sum_{j=0}^{t-1}\beta_j\limn\frac{\lL\bq^{t_1},\bq^j\lR}{\rho} &=& \limN \frac{\lL \bq^{t_1}, \bq^t_{||}\lR}{\rho},\label{eq:3.8a}\\
    &=& \limN \frac{\lL \bq^{t_1}, \bq^t_{||} \lR}{\rho} + \limN \frac{\lL \bq^{t_1}, \bq^t_{\perp} \lR}{\rho} ,\label{eq:3.8b}\\
    &=& \limN \frac{\lL \bq^{t_1}, \bq^t\lR}{\rho}, \label{eq:3.8c}
    \eeq 
    \end{subequations}
    where the \eqref{eq:3.8a} follows from the definition of $\bq^t_{||}$ in \eqref{eq:projection1b}, \eqref{eq:3.8b} follows from the fact that $\bq^j$ is orthogonal to $\bq^t_{\perp}$, for $j < t$, and \eqref{eq:3.8c} holds because $\bq^t = \bq^t_{\perp}+\bq^t_{||}$. 
    %%
    Thus, \eqref{eq:b2} holds when $t_1 < t$ and $t_2 = t$. 
    %%
    
    %%
    \noindent For $t_1 = t_2 =t$, the convergence $\limn \lL \bb^{t},\bb^{t} \lR$ is given by 
    \begin{subequations}
    \label{eq:3.9}
    \beq 
    \limn \lL \bb^t,\bb^t \lR &\ddis& \sum_{ i,j = 0}^{t-1}\beta_i\beta_j \limn  \lL\bb^i,\bb^j \lR + 2\sum_{i=0}^{t-1}\beta_i \limn\lL\bb^i, \widetilde{\bA}\bq^t_{\perp}\lR + \limn \lL\widetilde{\bA}\bq^t_{\perp},\widetilde{\bA}\bq^t_{\perp}\lR, \label{eq:3.9a} \\ 
    &\das&\sum_{ i,j = 0}^{t-1}\beta_i\beta_j \limn  \lL\bb^i,\bb^j \lR + \limn \lL\widetilde{\bA}\bq^t_{\perp},\widetilde{\bA}\bq^t_{\perp}\lR, \label{eq:3.9b}
    \eeq 
    \end{subequations} 
    where \eqref{eq:3.9a} follows from \eqref{eq:3.4} and \eqref{eq:3.9b} follows from the convergence in \eqref{eq:3.7}.
    %%
    %The first term in \eqref{eq:3.9b} can be rewritten as $\sum_{ i,j = 0}^{t-1}\beta_i\beta_j \limN  \frac{\lL\bq^i,\bq^j \lR}{\rho}$, which is a result of applying induction hypothesis to \eqref{eq:b2} for $i <t$ and $j < t$. 
    %%
    We now need to characterize the convergence of the term $\limn \lL\widetilde{\bA}\bq^t_{\perp},\widetilde{\bA}\bq^t_{\perp}\lR$ in \eqref{eq:3.9b}.
    %% 
    %%
    Applying {Proposition}~\ref{ps6} to $\widetilde{\bA}$ and $\bq^t_{\perp}$, the empirical distribution of $\widetilde{\bA}\bq^t_{\perp}$ converges to  
     $\widehat{\widetilde{\bA}\bq^t_{\perp}} \xRightarrow{d} \cN\bigg(0,\limN \frac{\lL\bq^t_{\perp},\bq^t_{\perp}\lR}{\rho}\bigg)$. 
     %% 
    Hence, the second moment of $\widehat{\widetilde{\bA}\bq^t_{\perp}}$ satisfies  
    \begin{equation}
    \label{eq:3.9.1}
    \limn \lL \widetilde{\bA}\bq^t_{\perp}, \widetilde{\bA}\bq^t_{\perp}\lR \das  \limN \frac{\lL\bq^t_{\perp},\bq^t_{\perp}\lR}{\rho}.
    \end{equation} Substituting \eqref{eq:3.9.1} into \eqref{eq:3.9b} gives 
    \begin{subequations}
    \label{eq:3.10}
    \beq 
    \limn \lL \bb^t,\bb^t \lR &\das& \sum_{ i,j = 0}^{t-1}\beta_i\beta_j \limn  \lL\bb^i,\bb^j \lR + \limN\frac{\lL\bq^t_{\perp},\bq^t_{\perp}\lR}{\rho}, \nonumber\\ 
    &\das&  \sum_{ i,j = 0}^{t-1}\beta_i\beta_j \limN  \frac{\lL\bq^i,\bq^j \lR}{\rho} + \limN\frac{\lL\bq^t_{\perp},\bq^t_{\perp}\lR}{\rho}, \label{eq:3.10b}\\
    &\das& \limN \frac{\lL\bq^t_{||},\bq^t_{||}\lR}{\rho} + \limN\frac{\lL\bq^t_{\perp},\bq^t_{\perp}\lR}{\rho}, \label{eq:3.10c}\\ 
    &\das& \limN\frac{\lL\bq^t,\bq^t\lR}{\rho}, \label{eq:3.10d}
    \eeq 
    \end{subequations}where \eqref{eq:3.10b} follows from applying induction hypothesis to \eqref{eq:b2} for $0 \leq t_1 = i, t_2 = j \leq t-1$. 
   %%
   The \eqref{eq:3.10c} and \eqref{eq:3.10d} follow from the definitions of $\bq^t_{||}$ in \eqref{eq:projection1b} and $\bq^t_{\perp}$ in \eqref{eq:projection2b}, respectively. 
   %%
   Therefore, \eqref{eq:b2} also holds for $t_1 =t_2 =t$, which completes the proof of \eqref{eq:b2} at the $t$th iteration.   \\
    %% \\
    d) Defining $\limN \frac{\lL \bq^t_{\perp}, \bq^t_{\perp}\lR}{\rho} \das \gamma^2_t$, then $\widehat{\widetilde{\bA}\bq^t_{\perp}} \xRightarrow{d} \cN(0,\gamma^2_t)$.
    Using the conditional distribution in \eqref{eq:3.4}, we get 
    \begin{equation}
        \label{eq:3.12}
        b^t_i|_{\cF_{t,t}} \xRightarrow{d} \sum_{j=0}^{t-1}\beta_jb^j_i + \gamma_tZ, \text{ for } i= 1,2,\dots,n,
    \end{equation}
     where $Z \sim \cN(0,1)$. 
     %%
     We define $\widetilde{\bu}^t_i = (b^0_i,\dots,b^{t-1}_i,\sum_{j=0}^{t-1}\beta_j b^j_i + \gamma_tZ,w_i)$, for $i= 1,2,\dots,n$.
     %%
     Then the convergence $\bu^t_i \xRightarrow{d} \widetilde{\bu}^ t_i$ holds due to \eqref{eq:3.12}, for $i= 1,2,\dots,n$. 
     %%
     To aprove \eqref{b:b}, we need to show that $\limn \frac{1}{n} \sumn \phi_b(\widetilde{\bu}^t_i) - \mathbb{E}\!\left[\phi_b(\sigma_0\widetilde{Z}_0,\dots, \sigma_t\widetilde{Z}_t, W)\right] \das 0$. By the triangular inequality,  
     %%
     \begin{equation}
         \label{eq:3.13}
         \bigg| \limn \frac{1}{n} \sumn \phi_b(\widetilde{\bu}^t_i) - \mathbb{E}\!\left[\phi_b(\sigma_0\widetilde{Z}_0,\dots, \sigma_t\widetilde{Z}_t, W)\right] \bigg| \leq X^t_1 + X^t_2, 
     \end{equation} 
     % $\bigg| \limn \frac{1}{n} \sumn \phi_b(\widetilde{\bu}^t_i) - \mathbb{E}\!\left[\phi_b(\sigma_0\widetilde{Z}_0,\dots, \sigma_t\widetilde{Z}_t, W)\right] \bigg| \leq X^t_1 + X^t_2$
     where $X^t_1$ $=$ $\bigg| \frac{1}{n}\sumn \bigg(\phi_b(\widetilde{\bu}^t_i) - \widetilde{\phi}_b(\bu^{t-1}_i)\bigg)\bigg|$, 
    $X^t_2$ $=$ $\bigg| \frac{1}{n}\sumn  \widetilde{\phi}_b(\bu^{t-1}_i) - \E[\phi_b(\sigma_0\widetilde{Z}_0,\dots,\sigma_t\widetilde{Z}_t,W)]\bigg|$, and $\widetilde{\phi}_b(\bu^{t-1}_i) = \E_{Z}[\phi_b(\widetilde{\bu}^t_i)]$, $\forall i$. 
    %%
    Similar to the proof of part d) in {Step}~1, we will verify that $\limn X^t_1 \das 0$ and $\limn X^t_2 \das0$. 
    %%
    
    %%
   First, the following holds due to \eqref{eq:controlled2}, 
   %%
   $|\phi_b(\widetilde{\bu}^t_i)| \leq c^t_{1} \exp\bigg[c^t_2\bigg(\sum_{j=0}^{t-1}|\beta_j b^j_i|^{\lambda} +\gamma^{\lambda}_t|Z|^{\lambda}+ |w_i|^{\lambda}\bigg)\bigg]$,  
   %%
   where $0<c^t_1$, $0< c^t_2$, and $1 \leq \lambda <2$ are constants. 
   %%
   Hence,
\begin{subequations}
\label{eq:3.14} 
\beq 
    \E_{Z}[|\phi_b(\widetilde{\bu}^t_i)|^{2+\kappa}] &\leq& c^t_{3} \exp\bigg[c^t_4\bigg(\sum_{j=0}^{t-1}|\beta_j b^j_i|^{\lambda} + |w_i|^{\lambda}\bigg)\bigg]\E_Z\bigg[\exp(c^t_4\gamma^{\lambda}_t|Z|^{\lambda})\bigg], \nonumber \\
    &=&c^t_5\exp\bigg[c^t_4\bigg(\sum_{j=0}^{t-1}|\beta_j b^j_i|^{\lambda} + |w_i|^{\lambda}\bigg)\bigg], \label{eq:3.14a}
\eeq 
\end{subequations} 
where $0< \kappa <1$, $c^t_3 = (c^t_1)^{2+\kappa}$, $c^t_4 = c^t_2(2+\kappa)$, and $c^t_5 = c^t_3\E_Z\bigg[\exp(c^t_4\gamma^{\lambda}_t|Z|^{\lambda})\bigg]$ are constants. 
%%
We define $X_{n,i} = \phi_b(\widetilde{\bu}^t_i) - \widetilde{\phi}_b(\bu^{t-1}_i) = \phi_b(\widetilde{\bu}^t_i) - \E_{Z}[\phi_b(\widetilde{\bu}^t_i)]$, for $i= 1,2,\dots,n$. 
%%
To prove the convergence $\limn X^t_1 \das 0$, we will show that $\{X_{n,i}\}_{i=1}^{n}$ satisfy the condition in {Lemma}~\ref{lm3}. 
%%
Indeed, the $\E_Z[|X_{n,i}|^{2+\kappa}]$ can be upper bounded as follows, 
%%
    \begin{subequations}
    \label{eq:3.15}
    \beq 
    \E_Z[|X_{n,i}|^{2+\kappa}] 
    &\leq&  2^{1+\kappa}\bigg[\E_Z\left[|\phi_b(\widetilde{\bu}^t_i)|^{2+\kappa}\right] + \left|\E_Z[\phi_b(\widetilde{\bu}^t_i)]\right|^{2+\kappa} \bigg], \label{eq:3.15b}\\ 
    &\leq & 2^{1+\kappa}\bigg[\E_Z\left[|\phi_b(\widetilde{\bu}^t_i)|^{2+\kappa}\right] + \E_Z\left[|\phi_b(\widetilde{\bu}^t_i)|^{2+\kappa}\right] \bigg], \label{eq:3.15c}\\ &=&2^{2+\kappa}\bigg[\E_Z\left[|\phi_b(\widetilde{\bu}^t_i)|^{2+\kappa}\right]\bigg] \leq  c^t_6\exp\bigg[c^t_4\bigg(\sum_{j=0}^{t-1}|\beta_j b^j_i|^{\lambda} + |w_i|^{\lambda}\bigg)\bigg],\label{eq:3.15e}
    \eeq 
    \end{subequations} 
    where  \eqref{eq:3.15b} follows from {Lemma}~\ref{lm4}, \eqref{eq:3.15c} follows from {Lemma}~\ref{lm5}, and \eqref{eq:3.15e} follows from \eqref{eq:3.14a} with $c^t_6 = 2^{2+\kappa}c^t_5$. 
    %%
    Defining $\psi_b(\bu^{t-1}_i) =  c^t_6\exp\bigg[c^t_4\bigg(\sum_{j=0}^{t-1}|\beta_j b^j_i|^{\lambda} + |w_i|^{\lambda}\bigg)\bigg]$, then $\psi_b(\bu^{t-1}_i)$ is a controlled function. The following holds,  
    \begin{subequations}
    \label{eq:3.16}
    \beq 
    \frac{1}{n}\sumn \E_{Z}[|X_{n,i}|^{2+\kappa}] &\leq& \frac{1}{n}\sumn \psi_b(\bu^{t-1}_i),\label{eq:3.16a}\\
    %%
    &\das& \E[\psi_b(\sigma_0\widetilde{Z}_0,\dots,\sigma_{t-1}\widetilde{Z}_{t-1},W)],\label{eq:3.16b}\\
    %%
    &<& cn^{\kappa/2},\text{for $n$ is sufficient large,}\label{eq:3.16c}
    \eeq 
    \end{subequations}
     where $c$ is a possitive constant,
     \eqref{eq:3.16a} follows from \eqref{eq:3.15e},
     \eqref{eq:3.16b} follows from applying induction hypothesis to \eqref{b:b} at $(t-1)$th iteration with $\psi_b(\bu^{t-1}_i)$, 
     and \eqref{eq:3.16c} holds because $\E[\psi_b(\sigma_0\widetilde{Z}_0,\dots,\sigma_{t-1}\widetilde{Z}_{t-1},W)] = c^t_7 < \infty$ while $ c^t_7 < cn^{\kappa/2}$ as $n_t < n$, for a constant $n_t$. 
    %%
    By {Lemma}~\ref{lm3}, the following convergence holds, $\limn \frac{1}{n}\sumn X_{n,i} \das 0$, implying 
    \begin{equation}
        \label{eq:3.17}
        \frac{1}{n}\sumn \bigg(\phi_b(\widetilde{\bu}^t_i) - \widetilde{\phi}_b(\bu^{t-1}_i)\bigg) \das 0, 
    \end{equation}
    which completes the proof of $\limn X^t_1 \das 0$.

     %%
     Now, showing $\limn X^t_2 \das 0$ is of interest. 
     %%
     Applying the induction hypothesis to \eqref{b:b} at $(t-1)$th iteration  with $\widetilde{\phi}_b(\bu^{t-1}_i)$ gives
    \begin{subequations}
    \label{eq:3.18}
    \beq 
    \limn \frac{1}{n} \sumn \widetilde{\phi}_b(\bu^{t-1}_i) &\das& \E[\widetilde{\phi}_b(\sigma_0\widetilde{Z}_0,\dots,\sigma_{t-1}\widetilde{Z}_{t-1},W)], \nonumber\\ 
    &=&\E\bigg[ \E_Z\bigg[\phi_b(\sigma_0\widetilde{Z}_0,\dots,\sigma_{t-1}\widetilde{Z}_{t-1},\sum_{j=0}^{t-1}\beta_j\sigma_j\widetilde{Z}_j + \gamma_tZ,W)\bigg]\bigg], \label{eq:3.18b} \\
    &=&\E\bigg[\phi_b(\sigma_0\widetilde{Z}_0,\dots,\sigma_{t-1}\widetilde{Z}_{t-1},\sum_{j=0}^{t-1}\beta_j\sigma_j\widetilde{Z}_j + \gamma_tZ,W)\bigg], \label{eq:3.18c}
    \eeq 
    \end{subequations}
    where \eqref{eq:3.18b} follows from the substitution $\widetilde{\phi}_b(\bu^{t-1}_i) = \E_{Z}[\phi_b(\widetilde{\bu}^t_i)]$. 
    %%
    Therefore, showing the convergence $\limn X^t_2 \das 0$ is equivalent to proving that $\sum_{j=0}^{t-1}\beta_j\sigma_j\widetilde{Z}_j + \gamma_tZ = \sigma_t\widetilde{Z}_t$, where $\widetilde{Z}_t \sim \cN(0,1)$ and $\sigma_t$ is defined in \eqref{eq:SE}. 
    %%

    %%
    \noindent In particular, for the controlled function $\phi_b(\bu^t_i) = (b^t_i)^2$, i.e.,  $\phi_b(\widetilde{\bu}^t_i) = \left(\sum_{j=0}^{t-1}\beta_jb^j_i + \gamma_tZ \right)^2$ because $\widetilde{\bu}^t_i = (b^0_i,\dots,b^{t-1}_i,\sum_{j=0}^{t-1}\beta_j b^j_i + \gamma_tZ,w_i)$, combining \eqref{eq:3.17} and \eqref{eq:3.18c} gives   
    %%
    \begin{equation}
        \label{eq:3.19}
        \limn \lL\bb^t,\bb^t \lR = \limn \frac{1}{n}\sumn \phi_b(\bu^t_i) \das \limn \frac{1}{n}\sumn \phi_b(\widetilde{\bu}^t_i) \das   \E\bigg[\bigg(\sum_{j=0}^{t-1}\beta_j\sigma_j\widetilde{Z}_j + \gamma_tZ\bigg)^2\bigg].
    \end{equation}
    %%    
    Applying \eqref{eq:b2} to $t_1=t_2=t$ leads to $\limn \lL\bb^t,\bb^t \lR \das \limN \frac{\lL\bq^t,\bq^t \lR}{\rho} = \sigma_t^2$, where the last equality holds because applying the induction hypothesis for $\phi_h(\bv^{t-1}_i) = f^2_t(h^{t}_i,x_{0i})$ in \eqref{b:h} gives $\frac{1}{\rho}\limN \lL \bq^t,\bq^t \lR \das \frac{1}{\rho}\E[f^2_t(\tau_{t-1}Z,X_0)] = \sigma^2_t$. 
    %%
    Hence, $\E\bigg[\bigg(\sum_{j=0}^{t-1}\beta_j\sigma_j\widetilde{Z}_j + \gamma_tZ\bigg)^2\bigg] \das \sigma^2_t$, implying $\sum_{j=0}^{t-1}\beta_j\sigma_j\widetilde{Z}_j + \gamma_tZ = \sigma_t\widetilde{Z}_t$ due to \eqref{eq:3.19}. 
    %%
    Thus, it is verified that $\limn X^t_2 \das 0$, which completes the proof of \eqref{b:b} at the $t$th iteration.           
    %%
    %%
    %%
    %%
    %%
    \subsection{Step 4: Conditioning on $\cF_{t+1,t} = \{\bb^0,\dots,\bb^{t},\bm^0,\dots,\bm^{t},\bh^1,\dots,\bh^t,\bq^0,\dots,\bq^t,\bx_0,\bw\}$.} 
    a) 
    Similar to part a) in {Step} 3, conditioning of $\bA$ on $\cF_{t+1,t}$ is equivalent to conditioning of $\bA$ on $\cP_{\bX_{t},\bY_{t+1}} = \{\bA|\bA^*\bM_{t} = \bX_{t}, \bA\bQ_{t+1} = \bY_{t+1}\}$. 
    %%
    Hence, applying Proposition~\ref{ps4} to characterize $\bA|_{\cF_{t+1,t}}$ and following the same procedure as in \cite[Lemma 1a]{Bayati11},  the $\bh^{t+1}|_{\cF_{t+1,t}}$ can be presented as 
    \begin{equation}
        \label{eq:4.1}
        \bh^{t+1}|_{\cF_{t+1,t}} \ddis \sum_{j=0}^{t-1}\alpha_j\bh^{j+1} +\widetilde{\bA}^*\bm^t_{\perp} - \bP_{\bQ_{t+1}}\widetilde{\bA}^*\bm^t_{\perp} + \bQ_{t+1}\overrightarrow{\bo}_t(1).
    \end{equation}
By {Proposition}~\ref{ps2}, we obtain $\limN \bP_{\bQ_{t+1}}\widetilde{\bA}^*\bm^t_{\perp} \das \mathbf{0}_N$. 
%%
In addition, we can verify that $\limN \bQ_{t+1}\overrightarrow{\bo}_{t}(1) \das \mathbf{0}_N$ by  characterizing the expectation and variance of the empirical distribution $\widehat{\bQ_{t+1}\overrightarrow{\bo}_{t}(1)}$ as $N \rightarrow \infty$. 
%%
Indeed,      
    \begin{equation}
        \limN |\lL \bQ_{t+1}\overrightarrow{\bo}_t(1) \lR| \leq  \limN  |o(1)|\frac{1}{N}\sumN \bigg|\sum_{j=0}^{t}q^j_i \bigg| \leq \limN |o(1)| \sum_{j=0}^{t} \frac{1}{N}\sumN |q^j_i| \das 0\label{eq:4.2},
    \end{equation}
    %%
    where the last estimation in \eqref{eq:4.2} holds because applying the induction hypothesis for $|q^j_i| = |f_j(h^{j}_i,x_{0i})|$  in \eqref{b:h} leads to $\limN \frac{1}{N}\sumN |q^j_i| \das \E[|f_j(\tau_{j-1}Z_{j-1},X_0)|] < \infty$, for $j<t+1$. 
    %%
    Hence, the  empirical expectation $ \lL \bQ_{t+1}\overrightarrow{\bo}_t(1) \lR$ converges to $0$, almost surely. 
    %%
    The empirical variance of $\widehat{\bQ_{t+1}\overrightarrow{\bo}_{t}(1)}$ converges to 
    \begin{subequations}
    \label{eq:4.3}
    \beq 
    \d4\d4\limN \lL \bQ_{t+1}\overrightarrow{\bo}_{t}(1)\lR_2 = \limN [o(1)]^2\frac{1}{N}\sumN \bigg(\sum_{j=0}^{t}q^j_i\bigg)^2 \d4 &\leq& \d4 \limN [o(1)]^2\frac{1}{N}\sumN (t+1) \sum_{j=0}^{t}(q^j_i)^2\label{eq:4.3b}, \\
    &=& \limN [o(1)]^2(t+1)\sum_{j=0}^t\lL\bq^j,\bq^j \lR \das 0\label{eq:4.3d},
    \eeq 
    \end{subequations} where \eqref{eq:4.3b}  follows from the Cauchy-Schwarz inequality and the last estimation in \eqref{eq:4.3d} holds because applying the induction hypothesis for $(q^j_i)^2 = f^2_j(h^{j}_i,x_{0i})$  in \eqref{b:h} leads to $\limN \lL\bq^j,\bq^j\lR \das \E[f^2_j(\tau_{j-1}Z_{j-1},X_0)] < \infty$, for $j <t+1$. Therefore, $\limN \bQ_{t+1}\overrightarrow{\bo}_{t}(1) \das \mathbf{0}_N$, implying that
    \begin{equation}
        \label{eq:4.4}
                \bh^{t+1}|_{\cF_{t+1,t}} \xRightarrow{d} \sum_{j=0}^{t-1}\alpha_j\bh^{j+1} +\widetilde{\bA}^*\bm^t_{\perp},
    \end{equation} which completes the proof of \eqref{eq:h1}.\\
    %%
    b) Applying \eqref{b:b} to $\phi_b(b^t_i,w_i) = g^{1+\alpha}_t(b^t_i,w_i)$ leads to $\limn \frac{1}{n} \sumn |m^t_i|^{2+2\alpha} \das \E[g^{2+2\alpha}_t(\sigma_t\widetilde{Z}_t,W)] < \infty$. Noting that $\sumn |m^t_{\perp i}|^{2+2\alpha} < \sumn |m^t_{i}|^{2+2\alpha}$, then the following holds $\limsupn \sumn |m^t_{\perp i}|^{2+2\alpha} < \infty$, which concludes \eqref{eq:alphaM}. \\
    %%
    c) For $t_1 <t$ and $t_2 =t$, the convergence $\limN \lL\bh^{t_1+1},\bh^{t+1}\lR$ is given by 
    \begin{subequations}
    \label{eq:4.5}
    \beq 
    \limN \lL \bh^{t_1+1},\bh^{t+1} \lR &\ddis& \limN \sum_{j=0}^{t-1}\alpha_j\lL\bh^{t_1+1},\bh^j\lR + \limN \lL\bh^{t_1+1},\widetilde{\bA}^*\bm^t_{\perp}\lR,\label{eq:4.5a}\\
    &\das& \sum_{j=0}^{t-1}\alpha_j\limn \lL\bm^{t_1},\bm^j\lR + \limN  \frac{\bm^{t^*}_{\perp}\widetilde{\bA}\bh^{t_1+1}}{N}. \label{eq:4.5b}
    \eeq 
    \end{subequations} 
    where \eqref{eq:4.5a} follows from \eqref{eq:4.4} and \eqref{eq:4.5b} follows from applying the induction hypothesis to \eqref{eq:h2} for $t_1 < t$ and $t_2=j < t$. 
    %%
    Now, we will specify the convergence of the second term in \eqref{eq:4.5b}, 
    %%
    %Applying {Proposition}~\ref{ps7} yields 
    %$\frac{\bm^{t^*}_{\perp}}{\|\bm^t_{\perp}\|_2} \widetilde{\bA} \frac{\bh^{t_1+1}}{\|\bh^{t_1+1}\|_2} \ddis \frac{Z}{\sqrt{n}}$, where $Z \sim \cN(0,1)$. Hence, the second term in \eqref{eq:4.5b} satisfies 
    \begin{subequations}
    \label{eq:4.6}
    \beq 
    \limN \frac{\bm^{t^*}_{\perp}\widetilde{\bA}\bh^{t_1+1}}{N}&=& \limN \frac{\|\bm^{t}_{\perp}\|_2 \|\bh^{t_1+1}\|_2}{N}\frac{\bm^{t^*}_{\perp}}{\|\bm^t_{\perp}\|_2} \widetilde{\bA} \frac{\bh^{t_1+1}}{\|\bh^{t_1+1}\|_2}, \label{eq:4.6a}\\
    &\ddis&\limN  \frac{\|\bm^{t}_{\perp}\|_2}{\sqrt{n}}\frac{\|\bh^{t_1+1}\|_2}{\sqrt{N}} \frac{\sqrt{n}}{\sqrt{N}}\frac{Z}{\sqrt{n}}, \label{eq:4.6b}\\
    &=&\sqrt{\rho}\limN \sqrt{\lL\bm^{t}_{\perp},\bm^{t}_{\perp} \lR \lL \bh^{t_1+1},\bh^{t_1+1}\lR}\frac{Z}{\sqrt{n}},\label{eq:4.6c}\\
    &\das& 0, \text{ for } t_1 < t, \label{eq:4.6d}
    \eeq 
    \end{subequations} 
    where \eqref{eq:4.6b} follows from applying Proposition~\ref{ps7} to $\frac{\bm^{t^*}_{\perp}}{\|\bm^t_{\perp}\|_2} \widetilde{\bA} \frac{\bh^{t_1+1}}{\|\bh^{t_1+1}\|_2}$, \eqref{eq:4.6d} follows because applying \eqref{eq:h2} for $t_1 < t+1$ leads to $\limN \lL \bh^{t_1+1},\bh^{t_1+1} \lR \das \limn \lL \bm^{t_1},\bm^{t_1} \lR < \infty$ and the convergence $\limn \lL\bm^t_{\perp},\bm^t_{\perp}\lR < \limn \lL \bm^t,\bm^t\lR < \infty$. 
    %%
    The last estimation holds because applying \eqref{b:b} for $\phi_b(b^t_i,w_i) = g^2_t(b^t_i,w_i)$ yields $\limN \lL \bm^t,\bm^t \lR \das \E[g^2_t(\sigma_t\widetilde{Z}_t,W)] < \infty$. 
    %%
    Substituting \eqref{eq:4.6d} into \eqref{eq:4.5b} yields
    \begin{subequations}
    \label{eq:4.7}
    \beq
     \limN \lL \bh^{t_1+1},\bh^{t+1} \lR  &=& \limn \lL\bm^{t_1},\sum_{j=0}^{t-1}\alpha_j\bm^j \lR = \limn \lL \bm^{t_1}, \bm^t_{||}\lR,\label{eq:4.7c}\\
     &=& \limn \lL \bm^{t_1}, \bm^t_{||}\lR + \limn \lL \bm^{t_1}, \bm^t_{\perp}\lR, \label{eq:4.7d}\\
     &=& \limn \lL \bm^{t_1}, \bm^t\lR, \label{eq:4.7e}
    \eeq 
    \end{subequations} 
    where \eqref{eq:4.7c} use the definitions of $\bm^t_{||}$ in \eqref{eq:projection1a} and \eqref{eq:4.7d} follows from the fact that $\bm^j$ is orthogonal to $\bm^t_{\perp}$, for $j < t$. Thus, \eqref{eq:h2} holds when $t_1 < t$ and $t_2 =t$.  
    %%%%%%%%%
    
    \noindent For $t_1 =t_2 = t$, the convergence $\limN \lL \bh^{t+1},\bh^{t+1} \lR$ is given by 
    \begin{subequations}
    \label{eq:4.8}
    \beq 
    \limN \lL \bh^{t+1},\bh^{t+1} \lR  &\ddis& \sum_{i,j = 0}^{t-1}\alpha_i\alpha_j \limN \lL \bh^{i+1},\bh^{j+1}\lR+2\sum_{i=0}^{t-1}\alpha_i\limN \lL\bh^{i+1},\widetilde{\bA}^*\bm^t_{\perp}\lR \nonumber \\ && + \limN \lL\widetilde{\bA}^*\bm^t_{\perp},\widetilde{\bA}^*\bm^t_{\perp}\lR, \label{eq:4.8a} \\
    &\das& \sum_{i,j = 0}^{t-1}\alpha_i\alpha_j  \limN \lL \bh^{i+1},\bh^{j+1}\lR + \limN \lL\widetilde{\bA}^*\bm^t_{\perp},\widetilde{\bA}^*\bm^t_{\perp}\lR, \label{eq:4.8b}
    \eeq 
    \end{subequations}
    where \eqref{eq:4.8a} follows from \eqref{eq:4.4} and  \eqref{eq:4.8b} follows from \eqref{eq:4.6d}. 
    %%
    %In \eqref{eq:4.8b} the first term can be represented by applying the induction hypothesis in \eqref{eq:h2} for $i <t $ and $j <t$ as $ \sum_{i,j = 0}^{t-1}\alpha_i\alpha_j \limn \lL \bm^{i},\bm^{j}\lR$. 
    %%
    We now need to characterize the convergence of the second term in \eqref{eq:4.8b}. 
    %%
    Applying {Proposition}~\ref{ps6} to $\widetilde{\bA}^*$ and $\bm^t_{\perp}$, the empirical distribution of $\widetilde{\bA}^*\bm^t_{\perp}$ converges to         $\widehat{\widetilde{\bA}^*\bm^t_{\perp}} \xRightarrow{d} \cN(0,\limn \lL \bm^t_{\perp},\bm^t_{\perp}\lR)$.
    %\begin{equation}
    %    \label{eq:4.9}     
    %\end{equation}
    Hence, the second moment of $\widehat{\widetilde{\bA}^*\bm^t_{\perp}}$ converges to 
    \begin{equation}
    \label{eq:4.10}
    \limN \lL\widetilde{\bA}^*\bm^t_{\perp},\widetilde{\bA}^*\bm^t_{\perp} \lR \das \limn \lL\bm^t_{\perp},\bm^t_{\perp}\lR. 
    \end{equation} Substituting \eqref{eq:4.10} into \eqref{eq:4.8b} leads to 
     \begin{subequations}
    \label{eq:4.11}
    \beq 
    \limN \lL \bh^{t+1},\bh^{t+1} \lR &\das& \sum_{i,j = 0}^{t-1}\alpha_i\alpha_j \limN \lL \bh^{i+1},\bh^{j+1}\lR+\limn \lL\bm^t_{\perp},\bm^t_{\perp}\lR, \label{eq:4.11a}\\
    &=&    \sum_{i,j = 0}^{t-1}\alpha_i\alpha_j \limn \lL \bm^{i},\bm^{j}\lR + \limn \lL\bm^t_{\perp},\bm^t_{\perp}\lR,\label{eq:4.11b}\\
    &=&\limn \lL\bm^t_{||},\bm^t_{||}\lR+\limn \lL\bm^t_{\perp},\bm^t_{\perp}\lR, \label{eq:4.11c} \\
    &=&\limn \lL \bm^t,\bm^t\lR \label{eq:4.11d}, 
    \eeq 
    \end{subequations}
    where \eqref{eq:4.11b} follows from applying induction hypothesis to \eqref{eq:h2} with $t_1 =i$ and $t_2 = j$, for $i<t,j<t$. 
    %%
    The \eqref{eq:4.11c} and \eqref{eq:4.11d} follows the definitions of $\bm^t_{||}$ in \eqref{eq:projection1a} and $\bm^t_{\perp}$ in \eqref{eq:projection2a}, respectively. Therefore, \eqref{eq:h2} also holds for $t_1 = t_2 =t$, which completes the proof of \eqref{eq:h2}.\\
    %%%% 
    d) Defining $\limn \lL \bm^t_{\perp},\bm^t_{\perp} \lR \das \Gamma^2_t$, then the empirical distribution $\widehat{\widetilde{\bA}^*\bm^t_{\perp}}$ converges,    \begin{equation}
    \label{eq:4.12}
            \widehat{\widetilde{\bA}^*\bm^t_{\perp}} \xRightarrow{d} \cN(0,\Gamma^2_t).
    \end{equation}
    Using \eqref{eq:4.12} and \eqref{eq:4.4}, the following convergence holds 
    \begin{equation}
        \label{eq:4.13}
          h^{t+1}_i|_{\cF_{t+1,t}} \xRightarrow{d} \sum_{j=0}^{t-1}\alpha_jh^{j+1}_i + \Gamma_tZ, \text{ for }i = 1,2,\dots,N,
\end{equation} 
where $Z \sim \cN(0,1)$. 
%%
Defining $\widetilde{\bv}^t_i = (h^1_i,\dots,h^{t}_i,\sum_{j=0}^{t-1}\alpha_jh^{j+1}_i + \Gamma_tZ,x_{0i})$, the convergence $\bv^t_i \xRightarrow{d} \widetilde{\bv}^t_i$ holds due to \eqref{eq:4.13}, for $i = 1,2,\dots,N$. Hence, to prove \eqref{b:h} we need to show that 
\begin{equation}
    \label{eq:4.14}
    \bigg|\limN \frac{1}{N}\sumN \phi_h(\widetilde{\bv}^t_i) - \E\bigg[\phi_h(\tau_0Z_0,\dots,\tau_tZ_t,X_0)\bigg] \bigg| \das 0.  
\end{equation} 
Similar to the proof of part d) in {Step}~2, following the triangular inequality, we verify \eqref{eq:4.14} by showing that $\limN Y^t_1 \das 0$ and $\limN Y^t_2 \das 0$, where
\begin{equation}
\label{eq:4.15}
Y^t_1 = \bigg|\frac{1}{N}\sumN \bigg(\phi_h(\widetilde{\bv}^t_i) - \widetilde{\phi}_h(\bv^{t-1}_i)]\bigg)  \bigg|,
\end{equation}
\begin{equation}
\label{eq:4.16.1}    
Y^t_2 = \bigg| \frac{1}{N}\sumN \widetilde{\phi}_h(\bv^{t-1}_i) - \E\bigg[\phi_h(\tau_0Z_0,\dots,\tau_tZ_t,X_0)\bigg] \bigg|,
\end{equation}
and $\widetilde{\phi}_h(\bv^{t-1}_i) = \E_Z[\phi_h(\widetilde{\bv}^t_i)]$, for $i=1,2,\dots,N$.
%%
The solution of $\limN Y^t_1 \das 0$ repeats the same procedure as in the  proof of $\limn X^t_1 \das 0$ in part d) of Step 3. 
%%
The detailed derivations are provided in Appendix B. 
%%
Noting that $\limn Y^t_1 \das 0$ is equivalent to
\begin{equation}
    \label{eq:4.15a}
    \limN \frac{1}{N}\sumN \bigg(\phi_h(\widetilde{\bv}^t_i) - \E_{Z}[\phi_h(\widetilde{\bv}^t_i)]\bigg) \das 0.
\end{equation} 

We are now readily to verify the convergence $\limN Y^t_2 \das 0$. Applying the induction hypothesis for $\widetilde{\phi}_b(\bv^{t-1}_i)$ in \eqref{b:h} gives 
\begin{subequations}
\label{eq:4.16}
\beq
    \limN \frac{1}{N}\sumN \widetilde{\phi}_h(\bv^{t-1}_i) &\das& \E[\widetilde{\phi}_h(\tau_0Z_{0},\dots,\tau_{t-1}Z_{t-1},X_0)],\label{eq:4.16a}\\
    &=&\E\bigg[\E_Z[\phi_h(\tau_0Z_{0},\dots,\tau_{t-1}Z_{t-1},\sum_{j=0}^{t-1}\alpha_j\tau_jZ_j+\Gamma_tZ,X_0)] \bigg],\label{eq:4.16b}\\
    &=&\E\bigg[\phi_h(\tau_0Z_{0},\dots,\tau_{t-1}Z_{t-1},\sum_{j=0}^{t-1}\alpha_j\tau_jZ_j+\Gamma_tZ,X_0) \bigg].\label{eq:4.16c} 
\eeq 
\end{subequations}Therefore, the rest of the proof for $\limN Y^t_2 \das 0$ is showing that $\sum_{j=0}^{t-1}\alpha_j\tau_jZ_j+\Gamma_tZ = \tau_tZ_t$, where $Z_t \sim \cN(0,1)$ and $\tau_t$ is defined in \eqref{eq:SE}.

For $\phi_h(\bv^t_i) = (h^t_i)^2$, i.e., $\phi_h(\widetilde{\bv}^t_i) = \left( \sum_{j=0}^{t-1}\alpha_jh^{j+1}_i + \Gamma_tZ \right)^2$ because $\widetilde{\bv}^t_i = (h^1_i,\dots,h^{t}_i,\sum_{j=0}^{t-1}\alpha_jh^{j+1}_i + \Gamma_tZ,x_{0i})$, combining \eqref{eq:4.15a} and \eqref{eq:4.16c} leads to 
\begin{equation}
    \label{eq:4.17}
    \limN \lL \bh^{t+1},\bh^{t+1} \lR = \limN \frac{1}{N}\sumN \phi_h(\bv^t_i) \das \limN \frac{1}{N}\sumN \phi_h(\widetilde{\bv}^t_i) \das  \E\bigg[\bigg(\sum_{j=0}^{t-1}\alpha_j\tau_jZ_j+\Gamma_tZ\bigg)^2\bigg].
\end{equation}
Using \eqref{eq:h2}, we get $\limN \lL \bh^{t+1},\bh^{t+1} \lR \das \limn \lL \bm^t,\bm^t \lR = \tau^2_t$, where the last equality holds because applying the induction hypothesis for $\phi_b(\bu^t_i) = g^2_t(b^t_i,w_i)$ in \eqref{b:b} yields $\limn \lL \bm^t,\bm^t \lR \das \E[g^2_t(\sigma_t\widetilde{Z}_t,W)] = \tau^2_t$. Hence, $\E\bigg[\bigg(\sum_{j=0}^{t-1}\alpha_j\tau_jZ_j+\Gamma_tZ\bigg)^2\bigg] \das \tau^2_t$ due to \eqref{eq:4.17}, which implies $\sum_{j=0}^{t-1}\alpha_j\tau_jZ_j+\Gamma_tZ = \tau_tZ_t$. Thus, it is  verified that $\limN Y^t_2 \das 0$, which completes the proof of \eqref{b:h} at the $t$th iteration.   
